Texture Memory-Augmented Deep Patch-Based Image Inpainting

Patch-based methods and deep networks have been employed to tackle image inpainting problem, with their own strengths and weaknesses. Patch-based methods are capable of restoring a missing region with high-quality texture through searching nearest neighbor patches from the unmasked regions. However, these methods bring problematic contents when recovering large missing regions. Deep networks, on the other hand, show promising results in completing large regions. Nonetheless, the results often lack faithful and sharp details that resemble the surrounding area. By bringing together the best of both paradigms, we propose a new deep inpainting framework where texture generation is guided by a texture memory of patch samples extracted from unmasked regions. The framework has a novel design that allows texture memory retrieval to be trained end-to-end with the deep inpainting network. In addition, we introduce a patch distribution loss to encourage high-quality patch synthesis. The proposed method shows superior performance both qualitatively and quantitatively on three challenging image benchmarks, i.e., Places, CelebA-HQ, and Paris Street-View datasets.

==> sections/__latexindent_temp.tex <==
% !TEX root = ../main.tex



\noindent
\textbf{Implementation Details.}
%
We follow the design of convolution blocks in PGGAN~\cite{karras2017progressive} to prepare our encoders and decoders as it proves to be effective on image generation. For all encoders in our T-MAD, a general downsampling block with `conv$3\times 3$, conv$3\times 3$, Downsample' is adopted and we halve the image resolution using nearest neighbor filtering. 
%
As for decoders in our framework, we apply `Upsample, conv$3\times 3$, conv$3\times 3$' as the basic building unit, named as upsampling block. The content-aware reassembly method, CARAFE~\cite{wang2019carafe}, is chosen as our `Upsample' method. 
%
In Tab.~\ref{tab:block}, we show the detailed number of the basic blocks in different modules. Note that we just apply a standard residual block~\cite{nazeri2019edgeconnect} in PSNet without any dilation operation. This is because PSNet aims at synthesizing high-quality textures at patch level and large receptive field is not necessary. In addition, we use leaky ReLU with leakiness 0.2 in all layers of the whole networks, except for the last layer in the decoder that uses linear activation.  We do not apply batch normalization or instance normalization in our T-MAD. In patch retrieval module, only two convolution layers with `conv$3\times 3$, conv$1\times 1$' are adopted for efficient feature extraction.

\begin{table}[t]
    \centering
    \caption{The number of basic blocks in different modules. `input-conv' and `out-conv' contain a $1\times 1$ convolution layer for channel transformation. `PSNet-FeatEnc' denotes the encoder in PSNet for extracting features from $\mathcal{T}_c$. The dilated residual block is denoted as `res-block'.}
    \vspace{-5pt}
    \begin{tabular}{c|c|c|c}
                & Coarse Net & PSNet-Backbone & PSNet-FeatEnc \\ \hline \hline
    input-conv  & 1              & 1              & 1             \\ \hline
    down-block  & 3              & 2              & 2             \\ \hline
    res-block   & 8              & 5              & 2             \\ \hline
    up-block    & 3              & 3              & 0             \\ \hline
    out-conv & 1              & 1              & 0            
    \end{tabular}
    \vspace{-8pt}
    \label{tab:block}
\end{table}

\begin{table}[tb]
    \centering
    \caption{Hyper-parameters in our T-MAD framework for random rectangle holes and free-form holes.}
    \vspace{-5pt}
    \label{tab:param}
    \small
    \begin{tabular}{c|c|c}
        \multicolumn{2}{c|}{}                            & Hyper-Parameters \\  \hline \hline
    \multirow{2}{*}{$\mathcal{L}_{\rm{recon}}$} & $\lambda_{\rm{valid}}$       & 1.         \\ \cline{2-3} 
                                      & $\lambda_{\rm{hole}}$        & 6.      \\ \hline
    \multirow{3}{*}{$\mathcal{L}_{\rm{ps}}$}    & $\lambda_{l_1}$          &  1.          \\ \cline{2-3} 
                                      & $\lambda_{\rm{gan}}^{pd}$    &    0.05       \\ \cline{2-3} 
                                      & $\lambda_{\rm{percep}}$      &     0.02      \\ \hline
    \multirow{2}{*}{$\mathcal{L}_{\rm{blend}}$} & $\lambda_{\rm{tv}}$          &    0.02       \\ \cline{2-3} 
                                      & $\lambda_{\rm{gan}}^{blend}$ &    0.02     
    \end{tabular}
    \vspace{-10pt}
\end{table}


\begin{table*}[tb]
    \centering
    \caption{The evaluation results of PatchMatch~\cite{barnes2009patchmatch}, GL~\cite{iizuka2017globally}, PICNet~\cite{zheng2019pluralistic}, Edge~\cite{nazeri2019edgeconnect}, StructureFlow~\cite{ren2019structureflow}, DeepFill~\cite{yu2018free} and CRA~\cite{yi2020contextual} over Places~\cite{zhou2017places} validation set. $\downarrow$ the lower the better, $\uparrow$ the higher the better. We report the inference speed for different methods on a single V100 GPU. $^\dagger$As we cannot obtain the original trained weights of GL, we re-implemented this method according to their paper \cite{iizuka2017globally}.}
    \vspace{-5pt}
    \begin{tabular}{c|c|c|c|c|c|ccccc|c|c}
     & \multicolumn{5}{c|}{random rectangle mask} & \multicolumn{5}{c|}{random irregular mask}  & \multicolumn{2}{c}{inference}                                                                           \\ \cline{2-13}
     & $l_1$ $\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & TV $\downarrow$ & FID$\downarrow$ & \multicolumn{1}{c|}{$l_1$ $\downarrow$} & \multicolumn{1}{c|}{PSNR$\uparrow$} & \multicolumn{1}{c|}{SSIM$\uparrow$} & \multicolumn{1}{c|}{TV $\downarrow$} & FID$\downarrow$ & FPS & \#param\\ \hline \hline
     PatchMatch     &14.795&15.038&0.819&\textbf{10.93}&11.630& \multicolumn{1}{c|}{11.276} & \multicolumn{1}{c|}{17.387} & \multicolumn{1}{c|}{0.839} & \multicolumn{1}{c|}{\textbf{13.02}} & 10.751 & 11 & -- \\
     GL$^\dagger$ &13.806&15.659&0.821&12.04&10.379& \multicolumn{1}{c|}{10.269} & \multicolumn{1}{c|}{17.403} & \multicolumn{1}{c|}{0.855} & \multicolumn{1}{c|}{13.50} & 8.295 & 24 & 3.6M \\
     PICNet &12.722&16.068&0.801&12.64&9.638 & \multicolumn{1}{c|}{9.477} & \multicolumn{1}{c|}{18.097} & \multicolumn{1}{c|}{0.860} & \multicolumn{1}{c|}{13.35} & 8.097 & 22 & 6.0M\\
     Edge&11.105&16.690&0.858&11.30&8.176& \multicolumn{1}{c|}{9.368} & \multicolumn{1}{c|}{18.249} & \multicolumn{1}{c|}{0.869} & \multicolumn{1}{c|}{13.44} & 8.097 & 20 & 5.3M \\
     StructureFlow&10.915&16.850&0.861&11.18&8.156& \multicolumn{1}{c|}{9.348} & \multicolumn{1}{c|}{18.279} & \multicolumn{1}{c|}{0.872} & \multicolumn{1}{c|}{13.24} & 8.080 & 18 & 10.2M \\
     DeepFill&10.829&16.843&0.859&11.35&8.148& \multicolumn{1}{c|}{9.372} & \multicolumn{1}{c|}{18.230} & \multicolumn{1}{c|}{0.871} & \multicolumn{1}{c|}{13.42} & 8.079 & 45 & 4.1M\\ 
     CRA&10.830&16.839&0.861&11.40&8.150& \multicolumn{1}{c|}{\textbf{9.260}} & \multicolumn{1}{c|}{18.226} & \multicolumn{1}{c|}{0.870} & \multicolumn{1}{c|}{13.33} & 8.071 & 48 & 2.7M\\ \hline 

     Our T-MAD &\textbf{10.334}&\textbf{17.203}&\textbf{0.867}&11.04&\textbf{8.131}& \multicolumn{1}{c|}{\textbf{9.261}} & \multicolumn{1}{c|}{\textbf{18.351}} & \multicolumn{1}{c|}{\textbf{0.873}} & \multicolumn{1}{c|}{13.27} & \textbf{8.058} & 47 & 3.9M
    \end{tabular}
    \label{tab:places}
    \vspace{-10pt}
\end{table*}


\begin{table}[tb]
    \centering
    \caption{The evaluation results of PatchMatch~\cite{barnes2009patchmatch}, PICNet~\cite{zheng2019pluralistic}, Edge~\cite{nazeri2019edgeconnect}, StructureFlow~\cite{ren2019structureflow}, and DeepFill~\cite{yu2018free} over CelebA-HQ and Paris Street-View validation set. $\uparrow$ the higher the better.}
    \vspace{-10pt}
    \begin{tabular}{c|c|c|cc}
     & \multicolumn{2}{c|}{CelebA-HQ} & \multicolumn{2}{c}{Paris Street-View}                                                                             \\ \cline{2-5}
     &  PSNR$\uparrow$ & SSIM$\uparrow$  & \multicolumn{1}{c|}{PSNR$\uparrow$} & SSIM$\uparrow$   \\ \hline \hline
     PatchMatch     &16.014&0.750& \multicolumn{1}{c|}{17.216}& 0.801 \\
     PIC     &25.210&0.852& \multicolumn{1}{c|}{25.620}& 0.834 \\
     Edge     &25.289&0.856& \multicolumn{1}{c|}{25.910}& 0.877 \\
     StructureFlow     &23.644&0.839& \multicolumn{1}{c|}{25.821}& 0.875 \\
     DeepFill     &	25.721 &0.871& \multicolumn{1}{c|}{26.012}& \textbf{0.881} \\ \hline 

     Our T-MAD &\textbf{26.138}&\textbf{0.882}& \multicolumn{1}{c|}{\textbf{26.153}} & 0.880
    \end{tabular}
    \label{tab:celeba-paris}
    \vspace{-20pt}
\end{table}



\begin{figure*}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/places-compare-cra.pdf}
    \vspace{-5pt}
    \caption{The qualitative comparison with existing models. From left to right: Corrupted input image, results of PatchMatch~\cite{barnes2009patchmatch}, PICNet~\cite{zheng2019pluralistic}, Edge-Connect~\cite{nazeri2019edgeconnect}, DeepFill~\cite{yu2018free}, CRA~\cite{yi2020contextual}, our T-MAD and ground-truth. (\textbf{Best viewed with zoom-in})}
    \label{fig:places-res}
    \vspace{-15pt}
\end{figure*}



To process patches in an efficient way within the existing deep learning framework for training, for each image, a fixed number $\mathbb{N}_{p_s}$ of $p_s$ are extracted and concatenated in an extra dimension. 
%
Once the number of actual masked patches is smaller than $\mathbb{N}_{p_s}$, we will randomly sample some valid patches from the unmasked region as complementary patches. As for testing, we can merely choose the masked patches to process in the patch synthesis stage.
%
In our experiments, we keep the patch size $k_p=32$. Because too small patches will cause boundary artifacts while large patches result in heavier training costs for obtaining a high-quality patch synthesis network.
%
The coarse network is pre-trained for four epochs to obtain a reasonable initialization for the following joint training procedure. 
%
%
In the joint training stage, we use four images in each batch and each image has different holes.
%
Note that PSNet adopts patches as input. The batch size for PSNet is equal to four times the number of hole patches in each image.
%
Thus, we do not need large image batches to perform adversarial training.
%
The whole model is trained on four Titan V GPUs for three days. 
%
In training, we use images of resolution $256 \times 256$ with the largest hole size $128\times 128$ in random positions. 
%
Cosine restart scheduler is also adopted as our training scheduler.
%
For each dataset mentioned below, we follow the official partition of the training and validation subsets.
%
% \revise{As for testing, given $256\times 256$ and $512\times 512$ inputs in V100, our method runs at 47 fps and 8 fps on average, respectively.}



As for the patch distribution loss described in Sec.~\ref{sec:psmodule}, we have the freedom of choosing  different $f$ and $g$ for the general formulation like ~\cite{jolicoeur2018relativistic}. In this paper, we apply classical non-saturated GAN loss in~\cite{goodfellow2014generative}. The hyper-parameters of losses are presented in Tab.~\ref{tab:param}.


%In Eq.~\eqref{eq:psgan-d} and Eq.~\eqref{eq:psgan-g}, we provide the general formulation and this formulation can be easily integrated in existing GAN models with only changing $f$ and $g$ for different kinds of methods. 
%
% We have integrated `Vanilla' and `WGAN-GP' like ~\cite{jolicoeur2018relativistic} into our patch distribution loss. Without special declaration, we use the model with `Vanilla' formulation in our experiments.
%
% However, the hyper-parameters are different in these two kinds of adversarial loss and we will specify them in the following sections.
%In Tab.~\ref{tab:param}, we present the hyper-parameters in T-MAD when applying different GAN losses.


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{figures/paris-compare-v2.pdf}
    \vspace{-10pt}
    \caption{Comparison of our model with PatchMatch~\cite{barnes2009patchmatch}, PIC~\cite{zheng2019pluralistic}, Edge-Connect~\cite{nazeri2019edgeconnect}, StructureFlow~\cite{ren2019structureflow}, and DeepFill~\cite{yu2018free} in Paris Street-View\cite{doersch2012what} validation set. (\textbf{Best viewed with zoom-in})}
    \label{fig:paris}
    \vspace{-10pt}
 \end{figure*}
 
 \begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{figures/celeba-compare-v2.pdf}
    \vspace{-10pt}
            \caption{Comparison of our model with PatchMatch~\cite{barnes2009patchmatch}, PIC~\cite{zheng2019pluralistic}, Edge-Connect~\cite{nazeri2019edgeconnect}, StructureFlow~\cite{ren2019structureflow}, and DeepFill~\cite{yu2018free} in CelebA-HQ validation set. (\textbf{Best viewed with zoom-in})}
    \label{fig:celeba}
    \vspace{-10pt}
 \end{figure*}

 \begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{figures/face-inpaint.pdf}
    \vspace{-15pt}
    \caption{Visualization for the face inpainting procedure with our T-MAD. In the patch retrieval stage, we only show the retrieved patch with the highest score.}
    \label{fig:face}
    \vspace{-15pt}
\end{figure}


\subsection{Main Results}

We evaluate the proposed T-MAD approach on three standard benchmarks Places~\cite{zhou2017places}, CelebA-HQ~\cite{karras2017progressive} and Paris Street-View~\cite{doersch2012what}. 
%
Among the three datasets, Places is the most challenging benchmark with more than 400 natural scenes of diverse objects and textures. 
%
CelebA-HQ and Paris Street-View comprise highly structured face and building images, respectively. 
%
Following the previous study~\cite{yu2018generative}, we use random rectangle masks with the same settings for evaluation. In addition, we also report results on Places with free-form irregular holes~\cite{yu2018free} to further demonstrate the effectiveness of T-MAD for handling various kinds of masks.



\noindent \textbf{Baselines.} We compare our methods with traditional optimization-based methods and contemporary deep inpainting methods:
\begin{itemize}
    \item PatchMatch~\cite{barnes2009patchmatch}: fills in the hole with the most optimal patches from unmasked regions.
    \item GL~\cite{iizuka2017globally}: introduces two discriminators to keep global and local consistency in the results.
    \item PICNet~\cite{zheng2019pluralistic}: introduce random noises for generating diverse results with deep generative network.
    \item Edge~\cite{nazeri2019edgeconnect}: adopts edge information to help reconstruct global structure.
    \item StructureFlow~\cite{ren2019structureflow}: applies the Relative Total Variation (RTV) map~\cite{xu2012structure} guiding the synthesis of global structure.
    \item DeepFill~\cite{yu2018free}: combines gated convolution and contextual attention module for high-quality results. To extract patches from unmasked regions, the contextual attention module adopts softmax function to fuse all of the features from valid regions.
    \item CRA~\cite{yi2020contextual}: improves DeepFill~\cite{yu2018free} with multi-scale contextual attention mechanism using shared attention scores.
\end{itemize}




\noindent\textbf{Quantitative Results.}
Following previous studies, we employ two kinds of metrics to measure distortion and perceptual quality, respectively. 
%
For distortion measurement, $l_1$ error, Peak Signal-to-Noise Ratio (PSNR), structural similarity index (SSIM), and total variation loss (TV loss) are adopted. %We expect that these four metrics can reflect the distortion from different views. 
%
As for the perceptual measurement, we use Fr\'{e}chet Inception Distance (FID)~\cite{heusel2017gans} to show the Wasserstein-2 distance between two distributions. %To some extent, it can indicate the perceptual quality of the results.
%
The evaluation results on Places validation set are reported in Tab.~\ref{tab:places}.
%
Except for GL~\cite{iizuka2017globally}, we directly use the released pre-trained weights and evaluate them in the same testing scheme.
%
The quantitative results of the baseline methods may be different from their papers, because we apply different testing schemes, e.g., the setting of mask ratios. 



%
The proposed T-MAD achieves competitive results compared with previous works. 
%
The better performance in PSNR and SSIM demonstrates that the patch-based generation can also contribute effectively to structural recovery. 
%
The lower FID score suggests our method is more effective in synthesizing realistic texture on such challenging dataset. It is noted that PatchMatch is doing better on TV metric because the method directly copies raw image patches. Although raw image patches bring a lower total validation loss, the overall structure in PatchMatch's results are not satisfactory.
%
For the inference speed, our T-MAD is even faster than the popular DeepFill methods. Without the time-consuming iterative optimization procedure used in PatchMatch, our texture memory and differentiable retrieval module can work in a more time-efficeint way. 


%     \footnote{As we cannot obtain the original trained weight, we re-implement this method according to their paper \cite{iizuka2017globally}.}



% \begin{figure*}[htb]
%     \centering
%     \includegraphics[width=\linewidth]{figures/paris-celeba.pdf}
%     \caption{Comparison of our model with PatchMatch~\cite{barnes2009patchmatch}, Edge-Connect~\cite{nazeri2019edgeconnect}, and DeepFill~\cite{yu2018free} on the Paris Street-View\cite{doersch2012what} and CelebA-HQ validation sets. (\textbf{Best viewed with zoom-in})}
%     \label{fig:paris-celeba}
%     % \vspace{-0.5cm}
% \end{figure*}


Besides, Tab.~\ref{tab:celeba-paris} provides quantitative comparisons on CelebA-HQ and Paris Street-View dataset. Since these two datasets contain few samples in the validation set, we only report the PSNR and SSIM metrics.
%
The competitive PSNR and SSIM in Tab.~\ref{tab:celeba-paris} prove the effectiveness of our T-MAD in such specific scenarios that contain highly structured patterns. 
%
We also observe that the performance of various methods in Places dataset is consistently worse than that in the other datasets, \ie, CelebA-HQ, and Paris StreetView.
%
A possible reason for this phenomenon is that CeleA-HQ and Paris StreetView only cover homogeneous domains within a single scenario, \ie, faces, or street views.
%
Nevertheless, Places dataset collects images from more diverse scenes and offers a larger validation set, which is more challenging in the inpainting task.





\noindent\textbf{Qualitative Results.}
Qualitative results are shown in Fig.~\ref{fig:places-res}. It is observed that the traditional patch-based method PatchMatch~\cite{barnes2009patchmatch} fills in the missing region with native texture patches but neglects the global structure. This is in concordance with its lower total variation loss but poorer performance on other metrics in Tab.~\ref{tab:places}.
%
Existing deep methods~\cite{nazeri2019edgeconnect,yu2018free,yi2020contextual} perform better structural recovery but the generated textures still suffer from artifacts.
%
On the contrary, our approach generates fine textures faithful to the unmasked regions, while obeying the global structure of the scene (\eg, the highly structured building in the second case). 
%
In addition, DeepFill~\cite{yu2018free} and CRA~\cite{yi2020contextual} both apply contextual attention mechanism to borrow information from valid regions, which is similar with our texture memory in some extent. However, they use a softmax function to fuse all of the features from unmasked regions and directly generate results at image level, which causes unnatural artifacts.
%
Thanks to the texture memory and patch synthesis, our T-MAD can easily handle more general cases in such large-scale dataset~\cite{zhou2017places}. 


\begin{table}[tb]
    \small
    \centering
    \caption{Ablation study on the number of candidates in the texture pool $\mathbb{N}_c$. `W-Sum' denotes fusing $\{p_c\}$ by simple weighted-sum with correspondance map $\mathcal{S}$. $\downarrow$ the lower the better, $\uparrow$ the higher the better}
    \vspace{-5pt}
    \begin{tabular}{c|c|c|c|c|c}
     & $l_1$ error$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & TV$\downarrow$ & FID$\downarrow$ \\ \hline \hline
     $\mathbb{N}_c = 1$ &10.341&17.119&0.852&11.52&8.151\\
     $\mathbb{N}_c = 2$ &10.336&17.130&0.859&11.46&8.147\\
     $\mathbb{N}_c = 4$ &\textbf{10.334}&17.203&\textbf{0.867}&\textbf{11.23}&8.131\\
     $\mathbb{N}_c = 6$ &10.335&\textbf{17.210}&0.864&11.24&\textbf{8.130}\\ \hline
     W-Sum        &10.602&16.872&0.853&11.31&8.602
    \end{tabular}
    \vspace{-10pt}
    \label{tab:nc}
\end{table}
\begin{figure}[tb]
    % \begin{minipage}{0.59\textwidth} 
    \includegraphics[width=\linewidth]{figures/pool.pdf}
    % \end{minipage}\hspace{0.01\textwidth}
    % \vspace{-15pt}
    % \begin{minipage}{0.38\textwidth} 
    \vspace{-10pt}
    \caption{We visualize the retrieval process of texture memory in the last column. The red color represents inpainted patches and other different colors represent the retrieval order of each $p_c^i$. For better visualization, we upsample the cropped patches}
    \label{fig:pool}
    \vspace{-5pt}
    % \end{minipage}
\end{figure}


Our method also achieves outstanding perceptual quality in comparison to other methods on highly structured street views (Fig.~\ref{fig:paris}) and faces (Fig.~\ref{fig:celeba}). Some interesting cases are observed.
%
For corrupted street views, benefiting from the texture memory, our approach learns to borrow similar textures from unmasked appearance of a building, leading to high-quality textures coherent with the original image. 


In masked faces, unlike PatchMatch, our model hallucinates reasonable and high-quality content for the missing parts.
%
Figure \ref{fig:face} presents the intermediate results in our T-MAD. 
%
The success is partially attributed to the structural guidance offered by the coarse network. The texture memory, interestingly, also functions very well despite the absence of highly identical patches from unmasked regions. The memory, in these examples, offers useful style information of the unmasked regions like complexion and facial texture for the completion. For the mouth patch in Fig.~\ref{fig:face}, PSNet encapsulates the ability of generating novel contents without the help of retrieved patches. Thus, out T-MAD can still achieve high-quality synthesis in such a challenging case.



\subsection{Ablation Study}

\noindent \textbf{Effectiveness of Texture Memory.}
Figure~\ref{fig:pool} presents two actual examples to show which texture patches $p_c^i\in \mathcal{T}_c$ are retrieved from the texture memory $\mathcal{T}$. 
%
Our approach tends to select patches with similar color or material from the texture memory $\mathcal{T}$.
%
In the first example of Fig.~\ref{fig:pool}, T-MAD retains a highly faithful texture recurrence with a reasonable semantic structure. It is interesting to see how texture synthesis can benefit from the statistical information provided by the texture memory $\mathcal{T}$.


\begin{figure}[t]
    % \begin{minipage}{0.59\textwidth} 
    \includegraphics[width=\linewidth]{figures/psgan-structure-revise.pdf}
    % \end{minipage}\hspace{0.01\textwidth}
    \vspace{-10pt}
    % \begin{minipage}{0.38\textwidth} 
    \caption{Ablation study on the Patch Distribution loss. Important regions are upsampled for detailed comparison. The first two samples are from Places with diverse scenes, while the last case contains more strctured textures from Paris Street-View. (\textbf{Best viewed with zoom-in})}
    \label{fig:pdloss}
    \vspace{-10pt}
    % \end{minipage}
\end{figure}

\begin{table}[tb]
    \caption{Quantitative results for our PSNet with standard GAN loss and our patch distribution loss. $\downarrow$ the lower the better, $\uparrow$ the higher the better}
    \small
    \centering
    \vspace{-5pt}
    \begin{tabular}{c|c|c|c|c}
                   & $l_1$ error $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & FID $\downarrow$ \\ \hline \hline
    w/ $\mathcal{L}_{\rm{gan}}$      &10.341&17.200&\textbf{0.869}&8.238\\ \hline
    w/ $\mathcal{L}_{\rm{gan}}^{pd}$ &\textbf{10.334}&\textbf{17.203}&0.867&\textbf{8.131}
    \end{tabular}
    \label{tab:pdloss}
    \vspace{-10pt}
\end{table}

\begin{figure}[t]
    % \begin{minipage}{0.59\textwidth} 
    \includegraphics[width=\linewidth]{figures/blend-ablation.pdf}
    % \end{minipage}\hspace{0.01\textwidth}
    % \vspace{-15pt}
    % \begin{minipage}{0.38\textwidth} 
    \vspace{-10pt}
    \caption{Ablation study on blending loss. (\textbf{Best viewed with zoom-in})}
    \label{fig:blend}
    % \end{minipage}
    \vspace{-15pt}
\end{figure}

\begin{figure*}[tb]
    
    \includegraphics[width=0.9\linewidth]{figures/multi-level-mod.pdf}
    \vspace{-5pt}
    \caption{Influence of mask size on inpainting methods. The first row depicts the input with mask showing in white. DeepFill~\cite{yu2018free} (second row) generates undesired artifacts when the area of missing region increases. In contrast, our method (last row) is still capable of synthesizing realistic textures (\textbf{Best viewed with zoom-in})}
    \label{fig:multilevel}
    \vspace{-15pt}
\end{figure*}



%\begin{figure}[tb]
%    \centering
%    \includegraphics[width=0.65\linewidth]{figures/pool.pdf}
%    \caption{We depict the retrieval process of texture memory in the last column. The red color represents inpainted patches and other different colors represent the retrieval order of each $p_c^i$. For better visualization, we upsample the cropped patches.}
%    \label{fig:pool}
%\end{figure}



The number of candidate texture patches $\mathbb{N}_c$ is a hyper-parameter in the texture retrieval module (Sec.~\ref{sec:pool}). We present the effect of different $\mathbb{N}_c$ in Tab.~\ref{tab:nc}. The `W-Sum' denotes fusing the texture pool with a simple weighted sum given the correspondence map $\mathcal{S}$.
%
We can clearly see that the weighted sum of texture pool harms the performance in both structure and texture. 
%
%Intuitively, the interpolation among different texture patches always leads to meaningless results. Even fusing similar texture patches with linear combination will cause blurry artifacts.
%
Selecting fewer texture patches slightly impairs the FID measurement, indicating lower quality of the generated textures. 
%
%From another perspective, this phenomenon further demonstrates the importance of our texture memory for that offers a diverse and helpful texture prior to PSNet.
%
We empirically found that increasing the number of texture patches beyond four does not bring more improvement as more repeated patches do not necessarily bring more statistical information of the unmasked region.
%Because the number of useful texture patches from the unmasked regions is limited, excessively increasing texture patches (more than four) brings no more improvement.



\noindent \textbf{Effectiveness of Patch Distribution Loss.}
%
An improved adversarial loss at patch level is introduced in Sec.~\ref{sec:psmodule}. 
%
Figure ~\ref{fig:pdloss} demonstrates the effectiveness of our Patch Distribution loss. We take the model without the relativistic components in Eq.~\eqref{eq:psgan-d} and Eq.~\eqref{eq:psgan-g} as the baseline for this ablation study, denoted by `$w/~\mathcal{L}_{gan}$' in Fig.~\ref{fig:pdloss} and Tab.~\ref{tab:pdloss}. 
%
We fix other modules and train only PSNet for a fair comparison. 
%
As shown in Fig.~\ref{fig:pdloss}, even though $\mathcal{T}$ contains useful texture patches, the model without patch distribution loss cannot learn to adopt the texture prior well. The case in Paris Street-View proves the effectiveness of patch distribution loss in synthesizing highly structured textures.
%
Furthermore, the quantitative results in Tab.~\ref{tab:pdloss} show that $\mathcal{L}_{\rm{gan}}^{pd}$ brings improvement in FID.
%
%However, thanks to the adversarial loss for patch distribution, our model is capable of effectively transferring existing texture prior to plausible synthesized results.
\begin{table}[tb]
    \caption{Quantitative results for our PSNet as a post-processing module in DeepFill~\cite{yu2018free} framework. $\downarrow$ the lower the better, $\uparrow$ the higher the better}
    \small
    \centering
    \begin{tabular}{c|c|c|c|c}
                   & $l_1$ error $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & FID $\downarrow$ \\ \hline \hline
    DeepFill       &10.829&16.843&0.854&8.148\\ \hline
    DeepFill+PSNet &\textbf{10.690}&\textbf{16.967}&\textbf{0.862}&\textbf{8.142}
    \end{tabular}
    \label{tab:post}
    \vspace{-10pt}
\end{table}

\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{figures/post-mod.pdf}
    % \vspace{-2pt}
    \caption{Effectiveness for applying our PSNet as post-processing module for DeepFill. Important regions have been upsampled for detailed comparison}
    \label{fig:post}
    \vspace{-15pt}
\end{figure}

\begin{figure*}[t]
    \centering
    % \includegraphics[width=\linewidth]{figures/irr-res.pdf}
    \includegraphics[width=0.9\linewidth]{figures/irr-mod.pdf}
    \caption{Application for object removal. In each example, from left to right: original image, masked image with white irregular holes and our results (\textbf{Best viewed with zoom-in})}
    \label{fig:object}
    \vspace{-15pt}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/supp_hr_new.pdf}
    \caption{Additional results for high-resolution input. The images shown in this figure are taken from Places val set with their original resolution. (\textbf{Best viewed with zoom-in})}
    \label{fig:supp-hr}
    \vspace{-15pt}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/failure-mod.pdf}
    % \vspace{-2pt}
    \caption{Failure cases of T-MAD}
    \label{fig:fail}
    \vspace{-15pt}
\end{figure*}

\noindent \textbf{Effectiveness of Blending Loss.}
To reduce boundary artifacts and preserve the local consistency between neighboring patches, a blending loss $\mathcal{L}_{blend}$ is adopted in our approach (Eq.~\eqref{eq:blendloss}). 
%
%Specifically, the total variation loss and the global patch discriminator guarantee the local consistency in final results.
%
We show its importance in our case study on CelebA-HQ.
%
As shown in Fig.~\ref{fig:blend}, inpainting without the blending loss is susceptible to complex light conditions as well as reflective property of human faces.
%
%Thanks to our blending loss $\mathcal{L}_{blend}$, our T-MAD can process separated patches in parrallel without worrying about the tiling artifacts.







\noindent \textbf{Influence of Mask Size.}
In Fig.~\ref{fig:multilevel}, we gradually increase the size of input mask to investigate the effects of mask size on inpainting methods. DeepFill~\cite{yu2018free} also adopts memory mechanism with Contextual Attention module. However, as the area of valid region reduces, the method cannot obtain useful information from unmasked regions while our T-MAD can make full use of a few selected patches to synthesize more realistic textures. Furthermore, the interpolation of texture representation in Contextual Attention module also causes undesired artifacts. On the contrary, our method performs better thanks to the more robust patch sampling (see Sec.~\ref{sec:pool}) in texture memory. %Importantly, our T-MAD synthesizes textures at patch level. When meeting extreme cases with masks spanning over the image (\eg last column in Fig~\ref{fig:multilevel}), it also leads to more competitive results than other methods that directly synthesize details on the entire image. 



\subsection{Applications}
\noindent \textbf{DeepFill + PSNet.}
As PSNet can also take inpainted images as the input, our patch synthesis module can be easily incorporated into recent inpainting models as a useful post-processing module. 
%
Taking DeepFill~\cite{yu2018free} method as an example, we adopt the results of DeepFill as input and fine-tune our PSNet with only 10,000 iterations.
%
As shown in Tab.~\ref{tab:post}, our PSNet improves the quantitative results with just a minor increase in computational cost. The inference time cost introduced by PSNet only accounts for 13\% over the total inference time.
%
Figure~\ref{fig:post} further demonstrates the effectiveness of PSNet as a post-processing module.
%
With the help of PSNet, DeepFill can better preserve local consistency in both structure and texture. 
%
Importantly, the more realistic textures in water and trees verify the importance of applying texture memory in image inpainting.

\noindent \textbf{Object Removal.}
Figure~\ref{fig:object} shows the examples of applying our method to object removal. Users can brush in arbitrary shapes and remove unwanted objects with our approach. The results suggest the generalizability of our approach in dealing with irregular missing regions.

\noindent \textbf{High-Resolution Result.}
To further show the effectiveness of T-MAD with high-resolution input, we present some challenging results in Fig.~\ref{fig:supp-hr}. Even if with high-resolution input ($512\times 768$), our methods can generate high-quality textures matching the original texture distribution.



\subsection{Failure Cases}

Some failure cases are shown in Fig.~\ref{fig:fail} for better understanding the limitation of our method. For most cases, the generated textures are reasonable but the global semantic structure are not fully recovered. It is because the coarse network fails to provide a faithful coarse result due to the complex scenes in the wild. In another failure case that is shown at the bottom-right of Fig.~\ref{fig:fail}, our method fails to hallucinate the whole body of the athlete due to the lack of semantic context.




==> sections/acknowledge.tex <==
\section{Acknowledgement}

